Modified Gravity and the Phantom of Dark Matter

Astrophysical data analysis of the weak-field predictions support the claim that modified gravity (MOG) theories provide a self-consistent, scale-invariant, universal description of galaxy rotation curves, without the need of non-baryonic dark matter. Comparison to the predictions of Milgrom's modified dynamics (MOND) provide a best-fit and experimentally determined universal value of the MOND acceleration parameter. The predictions of the modified gravity theories are compared to the predictions of cold non-baryonic dark matter (CDM), including a constant density core-modified fitting formula, which produces excellent fits to galaxy rotation curves including the low surface brightness and dwarf galaxies. Upon analysing the mass profiles of clusters of galaxies inferred from X-ray luminosity measurements, from the smallest nearby clusters to the largest of the clusters of galaxies, it is shown that while MOG provides consistent fits, MOND does not fit the observed shape of cluster mass profiles for any value of the MOND acceleration parameter. Comparison to the predictions of CDM confirm that whereas the Navarro-Frenk-White (NFW) fitting formula does not fit the observed shape of galaxy cluster mass profiles, the core-modified dark matter fitting formula provides excellent best-fits, supporting the hypothesis that baryons are dynamically important in the distribution of dark matter halos.

==> chapter/cluster/models/Gamma.tex <==
\subsection{\label{section.cluster.models.Gamma}Dynamic mass factor}



==> chapter/future/cosmo.tex <==
\section{\label{section.future.cosmo}Cosmology}
The seeded formation of the structure of galaxies and clusters of galaxies and precision measurements of the baryon-photon acoustic oscillations are derivable observations from the cosmic microwave background, and part of the subject of new experiments beyond WMAP.
\subsection{\label{section.future.cosmo.bbn}Baryogenesis and Leptogenesis}
\subsection{\label{section.future.cosmo.cmb}Cosmic microwave background}
\subsection{\label{section.future.cosmo.oscillations}Baryon photon acoustic oscillations}


==> chapter/galaxy/galaxy.tex <==
\section{\label{SECTION.GALAXY}Ursa Major filament of galaxies}

The Coma-Sculptor cloud surrounds the local group of the Milky Way, in the Virgo supercluster.  \citet{Tully.AJ.1996.112} identify 79 galaxies of the Ursa Major (UMa) filament, in the first of a trilogy of works, and provide surface brightness measurements in the blue, red and infrared bands.  UMa lies in the plane of the Virgo supercluster at the junction of filamentary structures, beyond the long axis of the filament of the Coma-Sculptor cloud.  \citet{Tully.APJ.1997.484} explore the differences in surface brightness amongst the 62 galaxies of the {\it complete sample}, and identify two distinct radial configurations of spiral galaxies of varying size, all of which are unevolved and rich in HI gas consistent with observations in Virgo and Fornax.  These are the high surface brightness (HSB) galaxies and the low surface brightness (LSB) galaxies.  Remarkably, even though the configurations differ, both types of HSB and LSB galaxies exhibit a common exponential disk for the central surface brightness profiles, described by the Van der
Kruit and Searle law, where the disk density distribution as a function of z (vertical height from the plane of the
disk) is given by
\begin{equation}
\label{eqn.galaxy.rotmodDisk}
\Sigma(z)={\rm sech}^{2}(z/z_{0})/z_{0},
\end{equation}
where $z_{0}$ is the vertical scale height of the luminous stellar disk, and is assumed to be 20\% of the near infrared
exponential disk scale length according to Column (13) of Table 2 of~\citet{Verheijen.APJ.2001.563}.

However, the mass to light ratio in LSB galaxies is difficult to explain using Newtonian gravity without dark matter dominated cores, whereas the mass to light ratio in HSB galaxies is difficult to explain using Newtonian gravity without baryon dominated cores and extended dark matter halos.  The UMa sample suggests that structure formation avoids the region of parameter space between  LSB and HSB galaxies, possibly due to different angular momentum regimes.  Passing from high  to low specific angular momentum, there is first the transition from LSB to HSB regimes, and at very low specific angular momentum, there is another transition from HSB galaxies which are exponential disk dominated to disk and bulge dominated.  Since the first transition can be modelled by a single parameter -- the mass to light ratio of the stellar exponential disk, whereas the second transition requires a second parameter -- the mass to light ratio of the bulge, we will focus exclusively on the subsample where the bulge can be neglected; and one parameter fits are possible for both HSB and LSB galaxies.  \citet{Sanders.APJ.1998.503} presented a third paper in the series on the rotation curves of UMa galaxies which focussed on the near-infrared band.  The existence of K-band surface photometry is a great advantage since the near-infrared
emission, being relatively free of the effects of dust absorption and less sensitive to recent star formation, is a more precise tracer of the mean radial distribution of the dominant stellar population.  The principal advantages of using infrared luminosities is that
stellar mass-to-light ratios are less affected by population differences and extinction corrections are
minimal~\citep{Verheijen.APJ.2001.563}.

\inserttable{table1}

For the sample of Ursa Major galaxies described in \tref{table.galaxy.uma}, it was observed that the exercise of fitting dark matter halos to galaxy rotation curve data requires three free parameters per galaxy -- the stellar disk mass to light ratio \(\Upsilon\), the halo density normalization \(\rho_0\), and core radius \(r_{s}\) -- tabulated in \tref{table.galaxy.coremodified}, and essentially any observed rotation curve can be reproduced.  It is important to note that \sref{section.conclusions.mog}{Solutions without dark matter} also produce excellent fits to the galaxy rotation curves, but in principle require only a single parameter, the stellar mass to light ratio, \(\Upsilon\), across the same sample of galaxies.

Whereas the singular halo models of \sref{section.halos.nfw}{Navarro-Frenk-White profile} produce acceptable fits to HSB galaxies, they generally fail for LSB galaxies.  \citet{McGaugh.APJ.1998.499} tested the dark matter hypothesis with LSB galaxies, finding that progressively lower surface brightness galaxies have progressively larger mass deficits, requiring high concentrations of dark matter deep in the galaxy core, rendering the visible components insignificant to the galaxy dynamics and leading to fine-tuning problems.  Conversely, the halo models of \sref{section.halos.coremodified}{Core-modified profile} fit all of the galaxies in the sample by means of the simple fitting formulae of \erefs{eqn.halos.coremodified}{eqn.halos.coremodified.mass}.

\subsection{\label{section.galaxy.velocity}Galaxy rotation curves}

The creation of galaxy rotation curves from astrophysical observations is subject to model dependent assumptions.  The road from photometry, in some observed electromagnetic band, to the surface mass density profile, in some chosen gravity theory, takes its way through the dynamics of the galaxy, with the destination a rotational velocity profile.  Spiral galaxies show a remarkable variation of the distribution and relative abundances of stellar material, distributed in bulges and disks, and the intergalactic medium, distributed in exponentially thin rings with vanishing amounts within galaxy cores.  These are the visible components --  the sources of photometric data -- that are used to reconstruct the dynamics of the galaxy, and the predicted galaxy rotation curves.

\insertfigure{fig1}

The method of generating the rotation curves closely followed \citet{Sanders.APJ.1998.503} and ~\citep{Verheijen.APJ.2001.563}.  The ROTMOD task of that group's Groningen Image Processing System (GIPSY)\footnote{\url{http://www.astro.rug.nl/~gipsy/}} was used to analyse the HI and K-band surface photometry data to produce the velocity profiles of the gaseous disk (HI plus He) distribution and luminous stellar disks, accounting for the \citet{Verheijen.AAP.2001.370} revised distance estimate to UMa from $D=15.5\,\mbox{Mpc}$ to $D=18.6\,\mbox{Mpc}$.

In order to measure each galaxy's mass to light ratio and produce galaxy maps, the stellar mass to light ratio, \(\Upsilon\), is treated as a free parameter, with results near unity considered reasonable. The baryon component velocities plotted in \fref{figure.galaxy.velocity} are based on the integrated surface mass density of the gaseous disk (HI plus He) component,
\begin{equation}
\label{eqn.galaxy.rotmodGas}
M_{\rm gas}(r) = \frac{4}{3} M_{\rm HI}(r),
\end{equation}
and luminous stellar disk component, \(M_{\rm disk}(r)\),
\begin{equation} \label{eqn.galaxy.baryonmass}
M_{\rm baryon}(r) = M_{\rm gas}(r) + \Upsilon M_{\rm disk}(r),
\end{equation}
listed in \tref{table.galaxy.coremodified}.  The dark matter halo velocities plotted in \fref{figure.galaxy.velocity} are based on the analytic fitting formula, \(M_{\rm halo}\), of \eref{eqn.halos.coremodified.mass} which is added to the baryonic mass to obtain the Newtonian dynamic mass,
\begin{equation} \label{eqn.galaxy.totalmass}
M_{\rm N}(r) = M_{\rm baryon}(r) + M_{\rm halo}(r).
\end{equation}

For each galaxy in the UMa sample, the total mass of \eref{eqn.galaxy.totalmass} is best-fit to the galaxy rotation curve data, through \eref{eqn.introduction.velocity}, by means of a non-linear least squares fitting algorithm, which minimizes the weighted sum of squares of deviations between the fit and the data.  The sum of squares of deviations is characterized by the estimated variance of the fit.  The reduced \(\chi^2/\nu\) statistic is computed as the value of \(\chi^2\) per degree of freedom,
\begin{equation} \label{eqn.galaxy.chi2}
\mbox{reduced}-\chi^2 \equiv \chi^2/\nu,\ \mbox{where}\ \nu=N-p,
\end{equation}
where the number of degrees of freedom, \(\nu\), is the difference between the number of data points in the galaxy rotation curve, \(N\), and the number of free parameters, \(p\).  The results are tabulated in \tref{table.galaxy.coremodified}.

\inserttable{table2}

\subsection{\label{section.galaxy.Sigma}Surface mass densities}

The importance of being able to determine the distribution of matter in astronomical objects is that it allows  predictions for ongoing and future experiments, such as gravitational lensing, which measures the line-of-sight surface mass density, 
\begin{equation}
\label{eqn.galaxy.Sigmarho}
\Sigma(r)\equiv\int \rho(r) dz,
\end{equation}
through the convergence,
\begin{equation}
\label{eqn.galaxy.kappa}
\kappa(r) = \frac{\Sigma(r)}{\Sigma_{c}},
\end{equation}
where \(\Sigma_{c}\) is the critical surface mass density~\protect\citep[Chapter 4]{Peacock:2003}.

\insertfigure{fig2}

The baryon component surface mass densities,
\begin{equation} \label{eqn.galaxy.baryonSigma}
\Sigma_{\rm baryon}(r) = \Sigma_{\rm gas}(r) + \Upsilon \Sigma_{\rm disk}(r),
\end{equation}
are determined by the stellar mass to light ratio, \(\Upsilon\), and the dark matter component, \(\Sigma_{\rm halo}(r)\), is determined by the central halo density, \(\rho_{0}\), and core radius, \(r_{s}\) -- all three parameters are fixed according to the best-fit algorithm of  \sref{section.galaxy.velocity} listed in \tref{table.galaxy.coremodified}.  The total surface mass density,
\begin{equation}
\label{eqn.galaxy.Sigmarho}
\Sigma(r)=\Sigma_{\rm baryon}(r) + \Sigma_{\rm halo}(r),
\end{equation}
is plotted in \fref{figure.galaxy.Sigma}.


It is important to notice that the surface mass densities combine to produce maps with features that can be traced back to the luminous stellar disk component for \(r<r_{s}\) and to the gaseous disk component for \(r \approx r_{s}\), whereas the dark matter halo dominates for \(r>r_{s}\).  The overall distribution is remarkably flattened in the galaxy core, as compared to the predictions of Newton's theory in the absence of dark matter.  Moreover, for every galaxy in the sample, the central surface mass density,
\begin{equation}
\label{eqn.galaxy.Sigma0}
\Sigma_0 \equiv \Sigma(0),
\end{equation}
is determined by the baryonic component alone, where the dark matter halo is rarified as a result of the core-modified model of \erefs{eqn.halos.coremodified}{eqn.halos.coremodified.mass}.  This is precisely the reverse situation for the singular halo models of \sref{section.halos.nfw}{Navarro-Frenk-White profile} which dominate the Newtonian dynamic mass throughout the galaxy, including the core.  Using the NFW profile leads to a situation where the baryon components may be everywhere neglected which erases the orphan features of the baryonic components discussed in \citet{Milgrom.APJ.2008.678}.  \citet{Kent.AJ.1986.91,Kent.AJ.1987.93,Kent.AJ.1988.96,Noordermeer.thesis.2006} provide arguments that galaxy rotation curves have distinct features that may be traced back to the luminous components.  The excellent fits -- plotted with orange solid lines -- in \fref{figure.galaxy.velocity} confirm that the baryonic components are dynamically important, but it is also shown that the Newtonian force law of \eref{eqn.introduction.newton} with only baryons -- plotted with brown dot-dotted lines -- fits none of the galaxy rotation curves outside the core.

\subsection{\label{section.galaxy.powerlaw}Power-law profiles}

The simple observation that galaxy rotation curves are approximately flat at large radii, where the orbital velocity of \eref{eqn.introduction.velocity} is constant, leads to the conclusion that the Newtonian dynamic mass of \eref{eqn.galaxy.totalmass} grows linearly with radius,
\begin{equation}\label{eqn.powerlaw.mass}
M_{N}(r) \propto r,
\end{equation}
and therefore, since we are not neglecting baryons,
\begin{equation}\label{eqn.powerlaw.rho}
\rho(r) \equiv \rho_{\rm baryon}(r) + \rho_{\rm halo}(r) \propto r^{-2},
\end{equation}
is valid where the galaxy rotation curves are approximately flat.  However, the radial distribution of spherically averaged dark matter halos is unlike either of the baryonic components which accumulate in exponentially thin HI (and He) gaseous disks or luminous stellar disks of \eref{eqn.galaxy.rotmodDisk}, and
\begin{eqnarray}
\label{eqn.powerlaw.galacticplane.on} &\rho_{\rm baryon}(r) \gg \rho_{\rm halo}(r)\ &\mbox{\tt on the galactic plane},\\
\label{eqn.powerlaw.galacticplane.off} &\rho_{\rm baryon}(r) \ll \rho_{\rm halo}(r)\ &\mbox{\tt off the galactic plane},
\end{eqnarray}

\insertfigure{fig3}

Therefore in order to generalize the power-law index of \eref{eqn.halos.coremodified.gamma} to include baryons, it is convenient to derive the relation using the spherically integrated power-law density of \eref{eqn.halos.powerlaw},
\begin{equation}\label{eqn.powerlaw.totalmass}
M_{N}(r) \propto \int_0^r \frac{ {r^{\prime}}^2}{{r^{\prime}}^{\gamma({r^{\prime}})}} d{r^{\prime}},
\end{equation}
and 
\begin{equation}\label{eqn.powerlaw.dtotalmass}
d M_{N}(r) \propto  {r}^{2-\gamma(r)} dr.
\end{equation}
Thus the spherically averaged power-law index may be defined in terms of the logarithm slope,
\begin{equation}\label{eqn.powerlaw.gamma}
\gamma(r) = 2 - \frac{d \ln M_{N}(r)}{d \ln r}.
\end{equation}
The power-law indices for the best-fit core modified halo and Newtonian dynamic mass including baryons of \erefs{eqn.halos.coremodified.gamma}{eqn.powerlaw.gamma}, respectively, are plotted in \fref{figure.galaxy.powerlaw}.

Since the virial radius of the halo naturally extends beyond the outermost radial point in the galaxy rotation curve, \(r_{\rm out}\), the dark matter to baryon fraction can grow without bound until the cosmological limit is reached.  Within each galaxy in the sample, the dark matter to baryon fraction is tabulated to the outermost radial point in the galaxy rotation curve -- in Column (8) of \tref{table.galaxy.coremodified} -- with mean values:
\begin{equation}\label{eqn.conclusion.dmfraction}
\frac{M_{\rm halo}(r_{\rm out})}{M_{\rm baryon}(r_{\rm out})} = \left\{ \begin{array}{ll} 2.4 \pm 2.1 & \mbox{\tt HSB galaxies}\\1.3 \pm 0.5 & \mbox{\tt LSB galaxies}\\2.0 \pm 1.8 & \mbox{\tt full sample}.\end{array}\right.
\end{equation}
which are consistently below the upper limit set by \citet{Spergel:ApJS:2007} in the Wilkinson microwave anisotropy probe (WMAP) third year results.



==> chapter/galaxy/tullyfisher.tex <==
\section{\label{section.galaxy.tullyfisher}The Tully-Fisher relation}

Whether galaxy rotation curves are best described by \sref{section.galaxy.dynamics.dm}, or \sref{section.galaxy.dynamics.mond}, or \sref{section.galaxy.dynamics.mog}, or other sensible theories, there are certain regularities in galactic structure which may have theoretical underpinning.

The luminosity radiated by a galaxy,
\begin{equation}
\label{eqn.galaxy.tullyfisher.luminosity} L = 4\pi \Phi d^2,
\end{equation}
may be inferred by measuring the isotropic flux, \(\Phi\), measured by terrestrial astronomy, and knowing the distance, \(d\), between earth and the galaxy. Since all of the galaxies in the sample of \sref{section.galaxy.uma} are at a common distance from the Milky Way, and because of the improvements identified in  \sref{section.galaxy.uma.photometry} from using the available near-infrared \(K\)-band, the large astronomical uncertainties are mitigated, leaving an ideal laboratory to study the relationship between the luminosity of a galaxy, and theoretical predictions from \sref{section.galaxy.dynamics}, for each gravity theory, independent of the galactic mass distribution and the existence of \sref{section.galaxy.halos}.

The observational \citet{Tully.AAP.1977.54} relation is an empirical correlation between the measured total luminosity of a galaxy in a particular band and the asymptotic rotational velocity of the form:
\begin{equation}
\label{eqn.galaxy.tullyfisher.relation} L \propto v_{\rm out}^{a} {\rm \ where\ } a \approx 3 - 4,
\end{equation}
where \(L\) is the total observed luminosity of the galaxy (in units
of \(10^{10} L_{\astrosun}\)), and \(v_{\rm out}\) is the observed velocity
at the outermost observed radial position (in km/s).  \cite{Tully.APJ.2000.533} showed that, although the exponent in \eref{eqn.galaxy.tullyfisher.relation} depends on the wavelength of the measured luminosity, and increases systematically from B to K bands, there appears to be convergence in the near-infrared where
\begin{equation}
\label{eqn.galaxy.tullyfisher.exponent} a = 3.4 \pm 0.1.
\end{equation}

\subsection{\label{section.galaxy.tullyfisher.velocity}The asymptotic velocity}

\citet{McGaugh.APJL.2000.533,McGaugh.APJ.2005.632} study a large sample of galaxies, with stellar masses ranging over five decades, and observe a change in slope in the Tully-Fisher relation which disappears when using the total baryonic mass including both stellar and gaseous components, instead of just the luminous stellar mass, and conclude that the Tully-Fisher relation is fundamentally a relation between the total baryonic mass and the rotational velocity.  Using a combination of \(K\)-band photometry and high resolution rotation curves, \cite{Noordermeer.MNRAS.2007.381} discover a second change in slope at the high mass end of the Tully-Fisher relation which disappears when using, in combination, the total baryonic mass and the asymptotic, outermost velocity instead of the maximum rotational velocity.

Considering the asymptotics of \fref{figure.galaxy.velocity}, the radial profiles are flat compared to the Newtonian predictions without non-baryonic dark matter, most high-resolution galaxy rotation curves are either slowly rising or slowly declining at large radii.  \citet{Verheijen.APJ.2001.563} considers an alternate definition of the ``flat rotation velocity'', \(v_{\rm flat}\), which categorizes galaxies according to three kinds of behaviour depending on the shape of the rotation curve.  The behaviour of \(v_{\rm out}\) is more closely related to the asymptotic ``flat rotation velocity''.

\cite{Avila-Reese.AJ.2008.136} explore the variation in the Tully-Fisher relation using a large sample of 76 high and low surface brightness galaxies, and confirm \eref{eqn.galaxy.tullyfisher.exponent} for the ordinary Tully-Fisher relation (where the stellar luminosity is taken proportional to the stellar mass), but that the value of the exponent in \eref{eqn.galaxy.tullyfisher.relation} may be as shallow as \(a=3.00\) for the baryonic Tully-Fisher relation, and \(a=2.77\) for the empirical \(B\)-band Tully-Fisher relation. 

\subsection{\label{section.galaxy.tullyfisher.ml}The mass luminosity relation}

Taking the logarithm of
both sides of \eref{eqn.galaxy.tullyfisher.relation}, we obtain
\begin{equation}\label{eqn.galaxy.tullyfisher.log} \log(L) = a \log(v_{\rm out}) + b.
\end{equation}
In order to calculate the total \(K\)-band luminosity,
apparent \(K\)-band magnitudes from the 2MASS survey were used.  Given an apparent \(K\)-band magnitude it is possible to calculate the \(K\)-band luminosity as
\begin{equation}
\label{luminosity}
\log_{10}(L_{K}) = 1.364 - \frac{2}{5} K_{T} + \log_{10}(1+z) + 2 \log_{10} D,
\end{equation}
where \(L_{K}\) is the \(K\)-band luminosity in units of \(10^{10} L_{\astrosun}\), \(K_{T}\) is the \(K\)-band apparent magnitude and z
is the
redshift of the galaxy (determined from the NASA/IPAC Extragalactic Database), and D is the distance to the galaxy in
Mpc.  The \(\log_{10}(1+z)\) term is a first order \(K\)-correction.  \citet[Figure 6]{Brownstein:ApJ:2006} plot the \(K\)-band observed Tully-Fisher relation based on a large sample of 101 LSB and HSB galaxies, in \fref{figure.galaxy.tullyfisher}, and determine empirically,
\begin{eqnarray}
\label{eqn.galaxy.tullyfisher.parameters} a_K &=& 2.85 \pm 0.33, \\
b_K &=& -5.73 \pm 0.74,
\end{eqnarray}
consistent with the results quoted above from \citet{Tully.APJ.2000.533,Avila-Reese.AJ.2008.136}.

As in \citet{Sanders.APJ.1998.503}, MOND is able to make predictions on both the slope and the intercept of the logarithmic Tully-Fisher relation by assuming that the stellar mass to light ratio, \(\Upsilon(r)\), is constant across all galaxies.  Although this is not the case, the assumption is enforced by using the best-fitting stellar mass to light ratio, \(\Upsilon\), to determine the values of the slope and intercept, \(a\) and \(b\), in \eref{eqn.galaxy.tullyfisher.log}. \fref{figure.galaxy.masslight} explicitly show the variation of the stellar mass to light ratio across each galaxy in the sample of \sref{section.galaxy.uma}, for each gravity theory, with the best-fitting, mean value is shown as a horizontal line.

Replacing the observed luminosity, \(L\), in the logarithmic Tully-Fisher relation of \eref{eqn.galaxy.tullyfisher.log} with
\begin{equation}
\label{eqn.galaxy.tullyfisher.mean} L = \frac{M}{\Upsilon},
\end{equation}
we obtain
\begin{equation}
\label{eqn.galaxy.tullyfisher.actual}
\log(M) = a \log(v_{\rm out}) + b - \log\left({\Upsilon}\right).
\end{equation}
Thus, the effect of \(\Upsilon\ne 1\) is to shift the \(\log(M)\)-intercept, \(b\); but does not affect the slope.  Theoretical predictions may be may quantified by either computing the appropriate \(\Upsilon\) values which depend on the particular band
of the luminosity measurements, or by considering the respective curve fits to the actual Tully-Fisher relation:
\begin{equation}\label{eqn.galaxy.tullyfisher.ab}
\log(M) = a \log(v_{\rm out}) + b.
\end{equation}
Taking the logarithm (with respect to base 10) of both sides of \eref{eqn.galaxy.dynamics.mond.vout }, we have the MOND predictions
\begin{eqnarray}
\label{eqn.galaxy.tullyfisher.parameters.a} a &=& 4, \\
\label{eqn.galaxy.tullyfisher.parameters.b} b &=& -8.21
\end{eqnarray}
If the Tully-Fisher relation is plotted using the MOND rotational velocity of \eref{eqn.galaxy.dynamics.mond.vout}; then the value of the logarithm slope of \eref{eqn.galaxy.tullyfisher.ab} will be precisely that of \eref{eqn.galaxy.tullyfisher.parameters.a}, tautologically.  In order to investigate the theoretical predictions of each gravity theory, the Tully-Fisher relation should be universally plotted using the values of the asymptotic velocity, \(v_{\rm out}\), from \tref{table.galaxy.uma}.

\fref{figure.galaxy.tullyfisher} plots the actual Tully-Fisher relation of \eref{eqn.galaxy.tullyfisher.ab} for the photometric fits, including the best-fit straight line.  In all cases, we are able to combine the HSB, LSB and  Dwarf galaxy data for the fitting, implying consistent physics across galaxies.  The numerical results of the respective fits are presented in \tref{table.galaxy.tullyfisher}.

\subsection{\label{section.galaxy.tullyfisher.mass}The galactic mass}


==> chapter/introduction/mog.tex <==
\subsection{\label{section.intro.mog}The alternative of modified gravity }
, and also here its twisted and offshell!

==> chapter/introduction/structure.tex <==
\subsection{\label{section.intro.structure}The process of structure formation}



%%%
The letter is divided as follows.  Section II provides recent results from studies of merging clusters of galaxies.  
The data from the Bullet Cluster is summarized, 
and the evidence for modified gravity is critically examined.

Section III presents some general issues on modified Friedmann Equations, Baryon-acoustic oscillation with a (general) running Newtonian constant, and provides 
recent results from theoretical simulations in modified gravity

==> macros.tex <==
%% MACROS
\newcommand{\slashpartial}{\displaystyle{\not} \partial}
\newcommand{\au}{\,\mbox{AU}}
\newcommand{\tbd}{\ldots}
\newcommand{\rc}{(r/r_{c})}
\newcommand{\SigmaN}{\Sigma_{c}}
\newcommand{\bc}{Bullet Cluster 1E0657-558}
\newcommand{\bul}{Bullet~1E0657-558}
\newcommand{\map}[1]{$#1$-map}
%% General Macros
\newcommand{\eprint}[1]{\href{http://www.arxiv.org/abs/#1}{arXiv:#1}}
%\renewcommand{\theenumi}{\roman{enumi}}
\newcommand{\cited}[1]{\protect\citep{#1}}
\newcommand{\citen}[1]{\protect\citet{#1}}
\newcommand{\physrep}{Phys.\,Rep.}
\newcommand{\eref}[1]{Equation (\ref{#1})}
\newcommand{\erefs}[2]{Equations (\ref{#1}) and (\ref{#2})}
\newcommand{\erefss}[3]{Equations (\ref{#1}), (\ref{#2}) and (\ref{#3})}
\newcommand{\erefsss}[4]{Equations (\ref{#1}), (\ref{#2}), (\ref{#3}) and (\ref{#4})}
\newcommand{\sfrac}[2]{\mbox{\small$\frac{#1}{#2}$}}
\newcommand{\half}{\mbox{\small$\frac{1}{2}$}}
\newcommand{\quarter}{\mbox{\small$\frac{1}{4}$}}
\newcommand{\sqrthalf}{\mbox{\small$\frac{1}{\sqrt{2}}$}}
\newcommand{\tcirc}[1]{\textcircled{\scriptsize #1}}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\vectprime}[1]{\mathbf{#1^{\prime}}}
\newcommand{\fbra}[2]{\langle \mbox{final}\,#1\,#2|}
\newcommand{\iket}[2]{|\mbox{initial}\,#1\,#2\rangle}
\newcommand{\bra}[1]{\langle #1|}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\braket}[2]{\langle #1|#2\rangle}
\newcommand{\mean}[1]{\langle #1\rangle}
\newcommand{\abs}[1]{\lvert#1\rvert} 
\newcommand{\norm}[1]{\lvert#1\rvert}
\newcommand{\dnorm}[1]{\lVert#1\rVert}
\newcommand{\vderiv}[1]{\frac{\delta}{\delta #1}}
\newcommand{\vvderiv}[2]{\frac{\delta #1}{\delta #2}}
\newcommand{\pderiv}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\creation}[1]{{\hat a}_{#1}^{\dagger}}
\newcommand{\annihilation}[1]{{\hat a}_{#1}}
\newcommand{\vectortwo}[2]{\left( 
\begin{array}{c}#1\\
#2
\end{array}\right)}
\newcommand{\hvectortwo}[2]{\Bigl(#1\quad#2\Bigr)}
\newcommand{\Hvectortwo}[2]{\biggl(#1\quad#2\biggr)}
\newcommand{\Vectortwo}[2]{\left( 
\begin{array}{c}#1\\ \\
#2
\end{array}\right)}
\newcommand{\matrixtwo}[4]{\left( 
\begin{array}{cc}#1&#2\\
#3&#4
\end{array}\right)}
\newcommand{\Matrixtwo}[4]{\left( 
\begin{array}{cc}#1&#2\\
\\
#3&#4
\end{array}\right)}
\newcommand{\Determinanttwo}[4]{\left| 
\begin{array}{cc}#1&#2\\
\\
#3&#4
\end{array}\right|}
\newcommand{\Identitytwo}{\left( 
\begin{array}{cc}1&0\\
\\
0&1
\end{array}\right)}
\newcommand{\rot}[2]{{\hat R}_{#2}(#1)}
\newcommand{\lab}[1]{#1_{{\rm Lab}}}
\newcommand{\zeff}{Z_{\mbox{eff}}}
\newcommand{\psirel}{\psi_{\mbox{rel}}}
\newcommand{\uvec}[1]{{\hat e}_{#1}}
\newcommand{\jay}{j}
\newcommand{\solar}{\odot}
%% Journal Abbreviations:
\newcommand{\nat}{Nature}
\newcommand{\pr}{Phys.\,Rev.}
\newcommand{\prl}{Phys.\,Rev.\,Lett.}
\newcommand{\prd}{Phys.\,Rev.\,D}
\newcommand{\plb}{Phys.\,Lett.\,B}
\newcommand{\jmp}{J.\,Math.\,Phys.}
\newcommand{\apj}{Astrophys.\,J.}
\newcommand{\apjl}{Astrophys.\,J.\,Lett.}
\newcommand{\apjs}{Astrophys.\,J.\,Suppl.\,Series}
\newcommand{\mnras}{Mon.\,Not.\,Roy.\,Astron.\,Soc.}
\newcommand{\araa}{Ann.\,Rev.\,Astron.\,Astrophys.}
\newcommand{\aap}{Astron.\,\& Astrophys.}
\newcommand{\aj}{Astron.\,J.}
\newcommand{\ijmpa}{Int.\,J.\,Mod.\,Phys.\,A.}
\newcommand{\ijmpd}{Int.\,J.\,Mod.\,Phys.\,D.}
\newcommand{\cqg}{Class.\,Quant.\,Gravity}
\newcommand{\cras} {Comptes Rendus Acad.\,Sci.}
\newcommand{\indicate}[1]{\begin{picture}(0, 0)\put(-18,22){\includegraphics{../Resources/png/icon/#1.png}}\end{picture}}
%% END MACROS


==> packages.tex <==
\usepackage{amsmath}\usepackage{amssymb}
\usepackage{fancyhdr}
\usepackage{setspace}
\usepackage{graphicx}% Include figure files
\usepackage{natbib}
\usepackage{makeidx}\makeindex
\usepackage{multicol}
\usepackage{pstricks}% Include figure files
\usepackage{lscape}
\usepackage{color}% \textcolor{color}{phrase}
\definecolor{LightMagenta}{cmyk}{0.1,0.8,0,0.1}
\definecolor{InkBlue}{rgb}{0.12,0.08,0.75}
\definecolor{InkYellow}{rgb}{0.8,0.42,0.42}
\definecolor{DarkBlue}{rgb}{0,0.08,0.45}
\definecolor{chocolate}{rgb}{0.2784,0.1216,0.1020}
\definecolor{orange}{rgb}{1.0,0.75,0}
\definecolor{DarkOrange}{rgb}{0.8,0.4,0}
\definecolor{DarkGreen}{rgb}{0.0,0.5,0.0}
\definecolor{shade}{rgb}{0.1,0.1,0.15}
\definecolor{sand}{rgb}{0.82,0.73,0.5}
\definecolor{cayenne}{rgb}{0.62,0.15,0.06}
\usepackage{wasysym}
\usepackage{caption}
\usepackage{multirow}
\usepackage[outercaption]{sidecap}
\captionsetup{justification=centerfirst,hangindent=8pt,singlelinecheck=false} 
\usepackage[pdftitle={Modified Gravity and the Phantom of Dark Matter},
			pdfauthor={J. R. Brownstein},
			pdfsubject={modified gravity, dark matter, bullet cluster, 1E0657-558, X-ray imaging, gravitational lensing},
			backref=page, bookmarks, bookmarksopen, bookmarksnumbered, 
%			colorlinks, linkcolor=black, citecolor=black, urlcolor=black]{hyperref}
			colorlinks, linkcolor=blue!97, citecolor=blue!97, urlcolor=blue!67!orange]{hyperref}

